Symmetric Sparse Boolean Matrix Factorization and Applications

In this work, we study a variant of nonnegative matrix factorization where we wish to find a symmetric factorization of a given input matrix into a sparse, Boolean matrix. Formally speaking, given $\mathbf{M}\in\mathbb{Z}^{m\times m}$, we want to find $\mathbf{W}\in\{0,1\}^{m\times r}$ such that $\| \mathbf{M} - \mathbf{W}\mathbf{W}^\top \|_0$ is minimized among all $\mathbf{W}$ for which each row is $k$-sparse. This question turns out to be closely related to a number of questions like recovering a hypergraph from its line graph, as well as reconstruction attacks for private neural network training. As this problem is hard in the worst-case, we study a natural average-case variant that arises in the context of these reconstruction attacks: $\mathbf{M} = \mathbf{W}\mathbf{W}^{\top}$ for $\mathbf{W}$ a random Boolean matrix with $k$-sparse rows, and the goal is to recover $\mathbf{W}$ up to column permutation. Equivalently, this can be thought of as recovering a uniformly random $k$-uniform hypergraph from its line graph. Our main result is a polynomial-time algorithm for this problem based on bootstrapping higher-order information about $\mathbf{W}$ and then decomposing an appropriate tensor. The key ingredient in our analysis, which may be of independent interest, is to show that such a matrix $\mathbf{W}$ has full column rank with high probability as soon as $m = \widetilde{\Omega}(r)$, which we do using tools from Littlewood-Offord theory and estimates for binary Krawtchouk polynomials.

==> compare.tex <==
\section{Comparison with Tensor Decomposition~\cite{adm+18}}
Symmetrc NMF problem can also be seen as a instance of the tensor decomposition problem.
Anari, Daskalakis,  Maass,  Papadimitriou, Saberi, and  Vempala \cite{adm+18} consider the tensor decomposition problem in an average instance.
\Runzhou{TODO} \Zhao{We need to list all the authors' last names}


==> connections.tex <==
\section{\Batched{} and Attacks on Federated Learning}
\label{app:grad}

Federated learning~\cite{mmrhy17,jdvebcdld16, jdekmrjmtv17, kjhyrsb16} is a popular machine learning scheme that is widely used when the training data is owned privately by multiple organizations. In this scheme, the different parties that participate in training only share gradient information about their respective data. Federated learning is believed to have a higher degree of privacy because the adversary can only observe stochastic gradients of the loss function arising from \emph{small batches of data}. However, there have been a number of empirical results showing that given such gradients, it is still possible to recover the private datasets \cite{zlh19, ymv+21, zmb20, wll+20, rg20}.

In this section, we make the observation that recovering the private datasets from these gradients is simply an instantiation of \Batched{}. Let ${\cal L}$ denote the loss function, and let $W \in\R^{m\times d}$ denote the weights in the first layer of the neural network being trained. As we show in Claim~\ref{cla:gradient_is_batched_k_sum}, when the network is feedforward with differentiable activations, the stochastic gradient vector computed from a batch of data points is essentially a linear combination of those data points.

The upshot is that if these batches are randomly chosen as in Assumption~\ref{assume:random} and we have access to an oracle for predicting similarity between gradients in the sense of Definition~\ref{defn:simmatrix_intro} (e.g. by training another neural network on labeled pairs of gradients), then we can successfully recover parts of the private datasets using our algorithm for \SSNMF{} together with the estimator in Section~\ref{sec:defer_recover_heavy}.

\subsection{ReLU Network Basics}

\begin{definition}[Feedforward network]
Consider a $L$ layer neural network with one vector $a\in \R^{m_L}$ and $L$ matrices $W_L \in \R^{m_L \times m_{L-1}}$, $\cdots$, $W_2 \in \R^{m_2 \times m_1}$ and $W_1 \in \R^{m_1 \times m_0}$. Let $m_0 = d$.
In order to write gradient in an elegant way, we define some auxiliary variables as follows
\begin{align}\label{eq:def_g_h}
g_{i,1} = & ~ W_1 x_i, && h_{i,1} = \phi(W_1 x_i), && \in \R^{m_1} && \forall i \in [n]\notag\\
g_{i,\ell} = & ~ W_{\ell} h_{i,\ell-1}, && h_{i,\ell} = \phi( W_{\ell} h_{i,\ell-1} ), && \in \R^{m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \\
%f(W,x_i) = & ~ a^\top h_{i,L}, && && \in \R && \forall i \in [n]\notag \\
D_{i, 1} = & ~ \mathrm{diag} \big(\phi'(W_1 x_i )\big), && && \in \R^{m_1 \times m_1} && \forall i \in [n] \notag\\
D_{i, \ell} = & ~ \mathrm{diag} \big(\phi'(W_{\ell} h_{i, \ell-1})\big), && && \in \R^{m_{\ell} \times m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \notag
%\label{eq:nn}
\end{align}
where $\phi(\cdot)$ is the activation function and $\phi'(\cdot)$ is the derivative of the activation function. 

The neural network $f: \R^{m_0}\to\R$ is given by the function
\begin{align*}
    f_W(x) = a^\top \phi( W_L ( \phi ( \cdots \phi(W_1 x ) ) ) ).
\end{align*}
In particular, using the definition of $h$ above, we have
\begin{align*}
    f_W(x_i) =  a^\top h_{i,L} \ \ \  \forall i \in [n]
\end{align*}
\end{definition}

\begin{definition}
Given a batch of $k$ input data points $(x_1 , y_1), \ldots, (x_k, y_k) \in \R^{d} \times \R$, define the loss $\mathcal{L}$ on those points by
\begin{align*}
\mathcal{L} (W) = \frac{1}{2} \sum_{i=1}^n ( y_i - f_W (x_i) )^2 .
\end{align*}
\end{definition}
 
\subsection{Close-form of the gradient}

We now show that the rows of the (matrix-valued) gradient of the $L_2$ loss over a batch of $k$ samples consists of linear combinations of 

\begin{claim}\label{cla:gradient_is_batched_k_sum}
Given a ReLU activated neural network, we consider training in the small batch setting with $n$ is the number of vectors in the batch. Let $x_1, \cdots, x_n \in \R^d$ denote those $n$ vectors in the small batch. Then each row of the gradient of the first layer weight can be written as a linear combination of $x_i$s, i.e.,
\begin{align*}
    (\frac{ {\cal L}(W) }{ \partial W_1})_{j,*} = \sum_{i=1}^n z_{j,i} x_i,
\end{align*}
where $z_{j,i}$ are coefficients.
\end{claim}
\begin{proof}

We can compute the gradient of ${\cal L}$ in terms of $W_{\ell} \in \R^{m_{\ell} \times m_{\ell-1}}$, for all $\ell \geq 2$
\begin{align}\label{eq:gradient}
\frac{\partial\mathcal{L}(W)}{\partial W_{\ell}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, \ell}}_{ m_{\ell} \times m_{\ell} } \left( \prod_{k = \ell+1}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{h_{i, \ell -1}^{\top}}_{1 \times m_{\ell-1}}
\end{align}
Note that the gradient for $W_1 \in \R^{m_1 \times m_0}$ (recall that $m_0 = d$) is slightly different and can not be written by a general form. Here is the form
\begin{align}
    \frac{\partial\mathcal{L}(W)}{\partial W_{1}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, 1}}_{ m_1 \times m_1 } \left( \prod_{k = 2}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{x_{i}^{\top}}_{1 \times m_{0}}
\end{align} 
\end{proof}

==> gradient.tex <==
\section{Recovering images from gradients is {\Batched}}
\label{sec:gradient_attack}

\iffalse
\subsection{One Hidden Layer}
We consider a one-hidden layer ReLU activated neural network with $m$ neurons in the hidden layer:
\begin{align*}
    f(x) = a^\top \phi(W x )
\end{align*}
where $a\in \R^m$ and $W \in \R^{m \times d}$.
We define objective function $L$ as follows:
\begin{align*}
    L(W) = \frac{1}{2} \sum_{i=1}^n (y_i - f(W,x_i,a))^2
\end{align*}
We can compute the gradient of $L$ in terms of $w_r$
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = \sum_{i=1}^n ( f(W,x_i,a) -y_i ) a_r x_i {\bf 1}_{ \langle w_r, x_i \rangle }
\end{align*}
Let $\wt{x} = \frac{1}{n} \sum_{i=1}^n x_i$,
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = ( f(W, \wt{x}, a) - y ) a_r \wt{x} {\bf 1}_{\langle w_r, \wt{x} \rangle}
\end{align*}
Another version
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = \sum_{i=1}^n ( f(W, x_i, a) - y_i ) \cdot \Big( a_r \wt{x} {\bf 1}_{\langle w_r, \wt{x} \rangle} \Big)
\end{align*}


\subsection{Two Hidden Layers}

Suppose $a \in \R^m$, $V \in \R^{m \times d}, W \in \R^{m \times m}$. The neural network is defined as $f : \R^d \rightarrow \R$, here we slightly deviate from the standard setting and assume the input dimension is $m$, in order to capture the general setting.
\begin{align*}
f(x) = a^{\top} \phi( W \phi ( V x ) )
\end{align*}
Consider the mean square loss
\begin{align*}
L(W, V, a) = \frac{1}{2} \sum_{i=1}^n | f(x_i) - y_i |^2
\end{align*}
The gradient with respect to $W$ is
\begin{align*}
\frac{ \partial L(W, V, a)}{ \partial W } = \sum_{i=1}^{n}(f(x_i) - y_i)  \underbrace{ \diag\{\phi'(W \phi(Vx_i))\} }_{ m \times m }\underbrace{ a }_{m \times 1}  \underbrace{ \phi(Vx_i)^{\top} }_{1 \times m}  
\end{align*}
and the gradient with respect to $V$ is
\begin{align*}
\frac{ \partial L(W, V, a)}{ \partial V } = \sum_{i=1}^{n}(f(x_i) - y_i)\underbrace{\diag\{ \phi'(Vx_i)\}}_{m \times m} \underbrace{W^{\top}}_{m \times m}  \underbrace{\diag\{\phi'(W \phi(Vx_i))\}}_{m \times m} \underbrace{a}_{m \times 1}    \underbrace{x_i^{\top}}_{1 \times d} 
\end{align*}

\subsection{The multi-layers case}
\fi



\subsection{Definitions}

The following multiple layer neural network definition is standard in the field of deep learning and machine learning. 

\begin{definition}[Multiple ReLU neural network]
Consider a $L$ layer neural network with one vector $a\in \R^{m_L}$ and $L$ matrices $W_L \in \R^{m_L \times m_{L-1}}$, $\cdots$, $W_2 \in \R^{m_2 \times m_1}$ and $W_1 \in \R^{m_1 \times m_0}$. Let $m_0 = d$.
In order to write gradient in an elegant way, we define some artificial variables as follows
\begin{align}\label{eq:def_g_h}
g_{i,1} = & ~ W_1 x_i, && h_{i,1} = \phi(W_1 x_i), && \in \R^{m_1} && \forall i \in [n]\notag\\
g_{i,\ell} = & ~ W_{\ell} h_{i,\ell-1}, && h_{i,\ell} = \phi( W_{\ell} h_{i,\ell-1} ), && \in \R^{m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \\
%f(W,x_i) = & ~ a^\top h_{i,L}, && && \in \R && \forall i \in [n]\notag \\
D_{i, 1} = & ~ \mathrm{diag} \big(\phi'(W_1 x_i )\big), && && \in \R^{m_1 \times m_1} && \forall i \in [n] \notag\\
D_{i, \ell} = & ~ \mathrm{diag} \big(\phi'(W_{\ell} h_{i, \ell-1})\big), && && \in \R^{m_{\ell} \times m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \notag
%\label{eq:nn}
\end{align}
where $\phi(\cdot)$ is the activation function and $\phi'(\cdot)$ is the derivative of the activation function. 

\end{definition}

We define the neural network as follows:
\begin{definition}
Let $f : \R^{m_0} \rightarrow \R$ denote neural network function: 
\begin{align*}
    f(W,x) = a^\top \phi( W_L ( \phi ( \cdots \phi(W_1 x ) ) ) )
\end{align*}
\end{definition}
Thus using the definition of $f$ and $h$, we have
\begin{align*}
    f(W,x_i) =  a^\top h_{i,L}, ~~~ \in \R, ~~~ \forall i \in [n]
\end{align*}

We use the standard $\ell_2$ loss here
\begin{definition}
Given $n$ input data points $(x_1 , y_1), (x_2 , y_2) , \cdots (x_n, y_n) \in \R^{d} \times \R$. We define the objective function $\mathcal{L}$ as follows
\begin{align*}
\mathcal{L} (W) = \frac{1}{2} \sum_{i=1}^n ( y_i - f (W,x_i) )^2 .
\end{align*}
\end{definition}
 

\subsection{Close-form of the gradient}

\begin{claim}\label{cla:gradient_is_batched_k_sum}
Given a ReLU activated neural network, we consider training in the small batch setting with $n$ is the number of vectors in the batch. Let $x_1, \cdots, x_n \in \R^d$ denote those $n$ vectors in the small batch. Then each row of the gradient of the first layer weight can be written as a linear combination of $x_i$s, i.e.,
\begin{align*}
    (\frac{ {\cal L}(W) }{ \partial W_1})_{j,*} = \sum_{i=1}^n z_{j,i} x_i,
\end{align*}
where $z_{j,i}$ are coefficients.
\end{claim}
\begin{proof}

We can compute the gradient of ${\cal L}$ in terms of $W_{\ell} \in \R^{m_{\ell} \times m_{\ell-1}}$, for all $\ell \geq 2$
\begin{align}\label{eq:gradient}
\frac{\partial\mathcal{L}(W)}{\partial W_{\ell}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, \ell}}_{ m_{\ell} \times m_{\ell} } \left( \prod_{k = \ell+1}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{h_{i, \ell -1}^{\top}}_{1 \times m_{\ell-1}}
\end{align}
Note that the gradient for $W_1 \in \R^{m_1 \times m_0}$ (recall that $m_0 = d$) is slightly different and can not be written by a general form. Here is the form
\begin{align}
    \frac{\partial\mathcal{L}(W)}{\partial W_{1}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, 1}}_{ m_1 \times m_1 } \left( \prod_{k = 2}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{x_{i}^{\top}}_{1 \times m_{0}}
\end{align} 
\end{proof}

==> instahide.tex <==
In this section we review the details about \Batched{} and its connection with \SSNMF. 
We defer the proof in section to Section~\ref{sec:instahide_defer}.% optimization problem \eqref{eq:factorization2}. %In lieu of ``feature vectors,'' we will refer to the elements of the private/synthetic datasets as ``images'' and their individual entries as ``pixels.''
%The main result of this section is to show the following:
We first give some definitions in \Batched{}.
%We first recall the process by which InstaHide generates synthetic images from private ones.
% We borrow heavily from the notation of \cite{clsz21}.

\begin{definition}[Original data matrix]
    Let  matrix $\X \in \R^{d \times n}$ be a matrix whose columns consist of vectors $\X_1,...,\X_n$ corresponding to $n$ vectors in $\R^d$. It will also be convenient to refer to the rows of $\X$ as $p_1,...,p_d\in\R^n$.
\end{definition}

\begin{definition}[{\Batched} synthetic data]
    Given matrix $\X$ and subset $S\subset[n]$ of size $k$, the corresponding \emph{synthetic data} is the vector $y^{\X,S}\triangleq \left|\sum_{i\in S} x_i\right|$
    % \begin{equation}\label{eq:instahide_def}
    %     y^{\X,S}\triangleq \left|\sum_{i\in S} x_i\right|,
    % \end{equation}
    where $|\cdot|$ denotes entrywise absolute value. We will refer to the vectors $\{x_i\}_{i\in S}$ as the \emph{constituent original vectors} of $y^{\X,S}$. To generate a \emph{synthetic dataset} of size $m$ via {\Batched}, one independently samples subsets $S_1,\ldots,S_m\subset[r]$ of size $k$ and outputs $\{y^{\X,S_1},...,y^{\X,S_m}\}$.
\end{definition}

% \Zhao{This needs rewording}
% The main finding of \cite{huang2020instahide} is that given a private dataset, one can train on the synthetic dataset generated by InstaHide and still achieve good test accuracy on the private dataset. The hope in that work was that taking the entrywise absolute value of $\sum_{i\in S} x_i$ makes it difficult to recover properties of the private images.

%\subsection{{\SSNMF} and {\Batched}}

% \iffalse
% As observed by \cite{clsz21,carlini_attack}, in many settings one can compute the matrix $\M'\in\R^{m\times m}$ whose $(i,j)$-th entry is $|S_i\cap S_j|$. Indeed, when the entries of the private image matrix $\X$ are independent Gaussians, then \cite{clsz21} gave a provable algorithm for extracting $\M'$ from the synthetic dataset. For real-world image datasets, when $k = 2$ in which case the entries of $\M'$ are $\{0,1\}$-valued, \cite{carlini_attack} gave a heuristic algorithm for computing $\M$ by training a neural network to classify pairs of synthetic images based on whether they have a constituent private image in common.
% \fi

We define the similarity between two sum vectors $y_i$ and $y_j$ to be $|S_i \cap S_j|$.
In real world, it is natural that we can use a neural network to predict the similarity between two $y_i$ and $y_j$. Therefore, it is natural to consider the \Batched{} problem with the following similarity oracle:

% For real-world image datasets and general $k$, while it is not necessarily so easy to recover $\M'$ itself with the latter strategy, as the entries of $\M'$ take values in $\{0,\ldots,k\}$ in general, it is nevertheless very plausible that one could still train a neural network to classify pairs of synthetic images as sharing at least one constituent private image or not. In other words, it is quite reasonable to assume access to the following matrix.

\begin{definition}[Similarity oracle]\label{defn:simmatrix}
    Given a synthetic dataset $\{y^{\X,S_1},\ldots,y^{\X,S_m}\}$ generated by \Batched, let ${\cal O}$ denote the oracle for which ${\cal O}(i,j) = |S_i\cap S_j| \neq \emptyset]$ for all $i,j\in[m]$.
    Also define the \emph{selection matrix} $\W\in\{0,1\}^{m\times r}$ to be the matrix whose $i$-th row is the indicator vector for subset $S_i$. Note that $\W$ is distributed as a matrix whose rows are independent random $k$-sparse Boolean vectors.
\end{definition}

The key property that relates \Batched{} to problem \eqref{eq:factorization2} is the following basic fact:

\begin{fact}\label{fact:tropicalfactorization}
    Let the matrix $\M \in \R^{m \times m}$ generated from ${\cal O}$ such that $\M_{i,j} = {\cal O}(i,j)$, then it satisfies $\M = \W\W^{\top}$.
\end{fact}
The above surprising fact tells us, as long as we have access to the similarity oracle ${\cal O}$, we do not need to have access to $\X$, to recover the selection matrix $\W$. In fact, we can even reconstruct $\X$.

\paragraph{Reconstructing $\X$ From a Factorization}

Suppose one can successfully construct the selection matrix $\W$ (up to column permutation) given similarity oracle ${\cal O}$. By definition of the synthetic dataset, we have that for any pixel index $j\in[d]$, if $z_j\in\R^m$ is the vector whose $i$-th entry is the $j$-th coordinate of $y^{\X,S_i}$, then $\W p_j = z_j.$ %\label{eq:system}


At this point is certainly information-theoretically possible to recover the original data matrix $\X$ by solving the linear systems.

% As for computationally efficient algorithms, note that \eqref{eq:system} can be thought of as an instance of \emph{phase retrieval} in a non-standard setting where the sensing matrix $\W$ consists of $k$-sparse binary measurements. \cite{hstzz20} showed that if $\W\in\calS_{m,r,k}$ is chosen adversarially instead of randomly, then this problem is computationally hard in general, even if $k = 2$. 

% When $\W$ is random as in Definition~\ref{defn:simmatrix}, the system \eqref{eq:system} appears to be easy to solve in practice. \cite{carlini_attack} demonstrated empirically in this case that when $\X$ is given by real-world image data, then one can efficiently solve \eqref{eq:system} by alternating minimization. In terms of provable algorithms, in \cite{clsz21}, the authors showed that if $m \ge r^{\Omega(k)}$, then with high probability over the choice of $\W$ there exists a submatrix of $\W$ of size $\binom{k + 2}{k}$ consisting of indicator vectors for all size-$k$ subsets of a particular set $T\subset[r]$ of size $k + 2$, and by brute-forcing over sign patterns for that particular collection of constraints in the piecewise-linear system \eqref{eq:system}, one can provably recover the coordinates of $p_j$ indexed by $T$ for any $j$. In other words, one can exactly recover the $k + 2$ images in the private dataset that are indexed by $T$. 

Here we give a different approach that allows us to recover the ``heavy'' coordinates of $p_j$ for any pixel index $j\in[d]$ that is faster than directly solve the linear system.



%\Zhao{The surprising part of the following lemma, we don't need matrix multiplication time and also we don't need access to database}
\begin{lemma}[Informal version of Lemma~\ref{lem:recoverheavy}]\label{lem:recoverheavy_intro}
    For any absolute constant $\eta > 0$, there is an absolute constant $c>0$ for which the following holds as long as $m \ge \Omega(\log(d/\delta))$. There is an algorithm {\sc GetHeavyPixels} that takes as input $\W$ defined according to Definition~\ref{defn:simmatrix} and vector $z$ satisfying $\W p = z$ for some vector $p\in\R^r$, runs in time $O(r\cdot m)$, and outputs $\wh{p}$ such that for every $i\in[r]$ for which $p_i \ge (ck/r)\cdot\overline{p}$, we have that $\wt{p}_i = p_i \cdot (1\pm \eta)$.
\end{lemma}

Using the above lemma, we have the following result:

\begin{theorem}[Informal version of Theorem~\ref{thm:instahide_formal}]\label{thm:instahide_formal_intro}
    For any absolute constant $\eta > 0$, there is an absolute constant $c > 0$ for which the following holds. Fix any integer $k \ge 2$, failure probability $\delta \in (0,1)$, and suppose $m \ge \widetilde{\Omega}(rk\log(d/\delta))$. Given a synthetic dataset of size $m$ generated by {\Batched} from a matrix $\X$, together with its similarity oracle, there is an $O(m^{\omega + 1} + d\cdot r\cdot m)$-time algorithm which outputs a matrix $\wh{\X}$ such that for any $(i,j)\in[r]\times[d]$ satisfying $|\X_{i,j}| \ge (ck/r)\sum_{i'\in[r]}|\X_{i',j}|$, we have that $|\wh{\X}_{i,j}| = |\X_{i,j}|\cdot (1 \pm \eta)$.
\end{theorem}

That is, we give a reconstruction algorithm that approximately recovers the magnitudes of the ``heavy'' indices of every vectors in the original data matrix, where an index $i$ is ``heavy'' if its value is roughly $k$ times larger in absolute value than the average value in that location across all original data vectors.

==> result.tex <==
%\subsection{Our results}

%In this section, we discuss our three results


%\paragraph{Worst case.}

%For the worst case, we provide a quasi-polynomial time algorithm (Theorem~\ref{thm:main_worst})
%\begin{theorem}\label{thm:main_worst}
%Given a matrix $\M = \W \W^\top \in \R^{m \times m}$ where each row of $\W \in \R^{m \times n}$ is a $k$-sparse binary vector, if $m \geq ???$ there is an algorithm that takes ??? time to output $\wt{\W} \in \R^{m \times n}$ such that
%\begin{align*}
%    \min_{\pi \in \Pi}\| \wt{\W} \pi \pi^\top \wt{\W}^\top - \W \|_F < ???
%\end{align*}
%where $\Pi \subset \R^{n \times n}$ is the set of all possible permutation matrices.
%\end{theorem}


%\paragraph{Average case.} For the average case, this problem become significantly easier, we provide two results (Theorem~\ref{thm:main_average} and Corollary~\ref{cor:main_average}). 
%\begin{theorem}\label{thm:main_average}
%Given a matrix $\M = \W \W^\top \in \R^{m \times m}$ where each row of $\W \in \R^{m \times n}$ is a random $k$-sparse binary vector, if $m \geq ???$ there is an algorithm that takes ??? time to output $\wt{\W} \in \R^{m \times n}$ such that
%\begin{align*}
%   \min_{\pi} \| \wt{\W} \pi \pi^\top \wt{\W}^\top - \W \|_F < ???
%\end{align*}
%where $\Pi \subset \R^{n \times n}$ is the set of all possible permutation matrices.
%\end{theorem}

%\Zhao{Ask sitan where to put this}

%\paragraph{Finite field.} In addition, the technique of our result in Theorem~\ref{thm:main_average} has the following application after doing some extra nontrivial calculations
%\begin{corollary}\label{cor:instahide_informal}
%Given a matrix $\M = \W \W^\top \in \mathbb{F}^{m \times m}$ where each row of $\W \in \mathbb{F}^{m \times n}$ is a random $k$-sparse binary vector, if $m \geq \Omega(n\log n)$ there is an algorithm that takes ??? time to output $\wt{\W} \in \mathbb{F}^{m \times n}$ such that
%\begin{align*}
%    \| \wt{\W} \wt{\W}^\top - \W \|_F < ???
%\end{align*}
%\end{corollary}

==> tensor.tex <==
\section{Average-Case Algorithm}
\label{sec:tensor}

In this section we prove Theorem~\ref{thm:avgcase}. Our algorithm is given by {\sc TensorRecover} below.

%\Zhao{Runzhou, please hardcode this algorithm as I explained to you before}
% \iffalse

% \fi

% In Section~\ref{subsec:formtensor}, we show how to construct the tensor $\T$ which is central to our algorithm. In Section~\ref{subsec:indep}, we prove a technical fact about the linear independence of the columns of $\W$. Finally, in Section~\ref{subsec:puttogether_tensor}, we put everything together and conclude the proof of Theorem~\ref{thm:avgcase}.








==> worst.tex <==
\section{Worst-case Algorithm}
\label{sec:worst}

In this section, we give a quasi-polynomial time algorithm for \eqref{eq:factorization2} in the worst case. We reduce the problem to solving a constraints satisfaction problem (CSP), and then use a 2-CSP solver developed by \cite{dm18} to find the solution. 


%Note that \cite{mm15} works for complete graph, in order to apply for our case, we need to convert our bipartite graph to complete graph by adding some trivial constraints (which will be true forever)


\iffalse
\newpage
\begin{table}[t]
    \centering
    \begin{tabular}{ |l|l|l|l|l| } \hline
        {\bf Refs} & {\bf Approx ratio} & {\bf Time} & {\bf Sol. exists} & {\bf Constructive} \\ \hline
        \cite{mm15} & $(1+\epsilon)$ & $(nq)^{O(\epsilon^{-1} \log n)}$ & Yes & Yes \\ \hline
        \cite{akk99} & $(1+\epsilon)$  & ? & No & Yes\\ \hline
        \cite{aim14} & $(1+\epsilon)$ & $qm\cdot (qn)^{O(\log(m)\cdot \epsilon^{-2})}$ & No & No\\ \hline
        \cite{bh17} & $(1+\epsilon)$ & $qm\cdot (qn)^{O(\log(m)\cdot \epsilon^{-2})}$ & No & No \\ \hline
        \cite{bhhs11} & ? & ? & ? & ?\\ \hline
        \cite{adkk03} & ?&?&?&?\\ \hline
        \cite{chk11} & $O((nq)^{1/3})$ & $\poly(n,q)$ & No & Yes\\ \hline
        \cite{mr17} &$1-\epsilon$ & $(nq)^{O(\epsilon^{-1}\cdot \log q)}$ & Yes & Yes\\ \hline
        \cite{y14} & additive $O(\epsilon)$ & $O(nq^4\cdot \epsilon^{-2})+q^{O(\epsilon^{-2}\cdot \log q)}$ & No & Yes\\ \hline
    \end{tabular}
    \caption{ $n$: number of variables; $q$:the size of the alphabet; For free game, the bipartite graph has $m$ vertices on the left and $n$ vertices on the right. Note their $q$ is our $\binom{r}{k}$.  We assume that the density of the CSP instance is $O(1)$.
    \cite{mr17} actually works for any $k$-CSP. \cite{y14} (Theorem~\ref{thm:theorem_1.2_in_y14}) is the fastest algorithm for 2-CSP, up to 2017. But the original paper has a wrongly claimed the running time of their algorithm, which was pointed out and corrected in \cite{mr17}.
    }
    \label{tab:upper_bound}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|l|l|} \hline
    {\bf Refs} & {\bf Approx ratio} & {\bf Time} & {\bf Assumptions} \\ \hline
    \cite{dm18} & $2^{(\log n)^{1/2+\rho}}\cdot n^{-1}~~v.s.~~ 1$ & $(nq)^{\omega(1)}$ & ETH, $\delta=1$\\ \hline
    \cite{dm18} & $2^{(\log n)^{1/2+\rho}}\cdot n^{-1} ~~v.s.~~ 1$ & $f(n)\cdot \poly(q)$ & Gap-ETH, $\delta=1$\\ \hline
    \cite{mr17} & $2^{-\widetilde{\Omega}(\log(nq))}~~v.s.~~1$ &$(nq)^{\omega(1)}$ & ETH, $\delta=1$ \\ \hline
    \cite{mr17} & $1/(nq)^{2/i}~~v.s.~~1$ & $(nq)^{\widetilde{\Omega}(i)}~~\forall i\geq i_0$ & ETAH, $\delta=1$ \\ \hline
    \end{tabular}
    \caption{$n$ variables and alphabet size $q$, density $\delta$. $f(n)$ is any function in $n$. Approx ratio shows the soundness v.s. the completeness. We use ETH to denote the Exponential Time Hypothesis. We use ETAH to denote the Exponential Time Hypothesis for Approximating Max 3SAT}
    \label{tab:lower_bound}
\end{table}

\subsection{QPTAS for Dense Max 2-CSPs}

%At first glance, it seems that the QPTAS would follow easily for our main theorem. This, however, is not the case as the algorithm in the main theorem always loses at least a constant factor. Instead, we need to give an algorithm that is similar to that of the main theorem but have a stronger guarantee in approximation ratio for satisfiable instances, which can be stated as follows. \\

\begin{lemma} \label{lem:approx-complete-game}
  For every positive integer $i > 0$, there exists an $(nq)^{O(i)}$-time algorithm that, for any satisfiable {\sc Max 2-CSP} instance on the complete graph, produces an assignment of value at least $1/q^{1/i}$.
\end{lemma}

%\Ruizhe{\cite{mr17} exactly recovered this result using Sherali-Adams Hierarch and independent rounding. They also gave a lower bound to show that this is almost tight, up to some $\poly\log i$ factors.}

%Lemma~\ref{lem:approx-complete-game} can be viewed as a special case of the main theorem when the graph is complete. However, it should be noted that Lemma~\ref{lem:approx-complete-game} is more exact in the sense that the guaranteed lower bound of the value of the output assignment is not asymptotic. The proof of this lemma is also similar to that of Lemma~\ref{lem:main} except that we need slightly more complicated algorithm and computation to deal with the fact that the underlying graph is not bipartite.

\begin{proof}[Proof of Lemma~\ref{lem:approx-complete-game}]
We will prove the lemma by induction. Note that throughout the proof, we will not worry about the randomness that the algorithm employs; it is not hard to see that the random assignment algorithms described below can be derandomized via greedy approach so that the approximation guarantees are as good as the expected guarantees of the randomized ones and that we still end up with the same asymptotic running time.

Let $P(i)$ represent the following statement: there exists an $O\left((nq)^{3i}\right)$-time algorithm {\sc Approx-CompleteGame$_i$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_u\}_{u \in V}$) that takes in a satisfiable {\sc Max 2-CSP} instance 
\begin{align*}(q, V, E, \{C_{e}\}_{e \in V})
\end{align*}
where $(V, E)$ is a complete graph and a reduced alphabet set $S_u$ for every $u \in V$ such that, if $\sigma^{\OPT}_u \in S_u$ for every $u \in V$, then the algorithm outputs an assignment of value at least $\left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{\frac{1}{ni}}$.

Observe that $P(i)$ implies the lemma by simply setting $S_u = [q]$ for every $u \in V$.

\paragraph{Base Case.} The algorithm {\sc Approx-CompleteGame$_1$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_u\}_{u \in V}$) is a simple random assignment algorithm. However, before we randomly pick the assignment, we need to first discard the alphabets that we know for sure are not optimal. More specifically, {\sc Approx-CompleteGame$_1$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_u\}_{u \in V}$) works as follows.

\iffalse
\begin{algorithm}[h]\caption{}
\begin{algorithmic}[1]
\Procedure{$\textsc{ApproxCompleteGame}_0$}{$\Sigma, V, E, \{C_{e}\}_{e \in E}, \{S_u\}_{u \in V}$}
    \While{$\exists u, v \in V$ and $\sigma_u \in S_u$ s.t. $ C_{(u, v)}(\sigma(u), \sigma(v)) = 0, \forall \sigma_v \in S_v$}
        \State $S_u \leftarrow S_u \backslash \{ \sigma(u) \};$
    \EndWhile
    \For{$u \in V$}
        \State pick $\varphi(u)$ independently and uniformly at random from $S_u$.
    \EndFor
    \State {\bf return} $\varphi$.
\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi
\begin{itemize}
  \item {\bf Step 1.} While there exist $u, v \in V$ and $\sigma_u \in S_u$ such that 
  \begin{align*}
      C_{(u, v)}(\sigma_u, \sigma_v) = 0, \forall \sigma_v \in S_v
  \end{align*}
  then remove $\sigma_u$ from $S_u$. \label{step:remove}
  \Ruizhe{This step doesn't work for matrix factorization. No matter what $A_{u,v}$ is, as long as $k$ is small, for any $k$-sparse vector $\sigma_u\in \F_2^r$, there will always exist a $k$-sparse vector $\sigma_v\in \F_2^r$ such that $\langle \sigma_u,\sigma_v\rangle=A_{u,v}$. 
  
  So, no $\sigma_u$ will be removed.}
  \item {\bf Step 2.} For each $u \in V$, pick $\varphi(u)$ independently and uniformly at random from $S_u$. Output $\varphi$.
\end{itemize}

It is obvious that the algorithm runs in $O(n^3q^3)$ time as desired. \Ruizhe{$O(n^2q^2)$ is enough.}

Now, we will show that,
\begin{claim} 
If $\sigma_u^{\OPT} \in S_u$ for every $u \in V$, then the algorithm gives an assignment that is of value at least $\left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{\frac{1}{n}}$ in expectation.
\end{claim}

First, observe that $\sigma_u^{\OPT}$ remains in $S_u$ after step \ref{step:remove} for every $u \in V$. This is because \begin{align*}
    C_{(u, v)}(\sigma_u^{\OPT}, \sigma_v^{\OPT}) = 1, \forall v \neq u.
\end{align*}

Next, Consider the expected number of satisfied edges by the output assignment, which can be rearranged as follows:
\begin{align*}
  \mathbb{E}\left[\sum_{(u, v) \in E} C_{(u, v)}(\varphi(u), \varphi(v))\right] &= \sum_{(u, v) \in E} \mathbb{E}\left[C_{(u, v)}(\varphi(u), \varphi(v))\right] \\
  &= \sum_{(u, v) \in E} \frac{1}{|S_u||S_v|} \sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v). \\
\end{align*}

From the condition of the loop in step~\ref{step:remove}, we know that after the loop ends, for each $\sigma_u \in S_u$, there must be at least one $\sigma_v \in S_v$ such that $C_{(u, v)}(\sigma_u, \sigma_v) = 1$. In other words, $$\sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v) \geq \sum_{\sigma_u \in S_u} 1 = |S_u|.$$

Similarly, we can also conclude that $$\sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v) \geq |S_v|.$$

Thus, we have $$\sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v) \geq \max\{|S_u|,|S_v|\}$$ for every $u \neq v$.

Hence, we can bound the expected number of satisfied edges as follows:
\begin{align*}
  \sum_{(u, v) \in E} \frac{1}{|S_u||S_v|} \sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v)
  &\geq \sum_{(u, v) \in E} \frac{1}{|S_u||S_v|} \max\{|S_u|, |S_v|\} \\
  &= \sum_{(u, v) \in E} \frac{1}{\min\{|S_u|, |S_v|\}} \\
  &\geq \sum_{(u, v) \in E} \frac{1}{\sqrt{|S_u||S_v|}} \\
  (\text{A.M. - G.M. inequality}) &\geq |E| \left(\prod_{(u, v) \in E} \frac{1}{\sqrt{|S_u||S_v|}}\right)^{\frac{1}{|E|}} \\
  &= |E| \left(\prod_{(u, v) \in E} \frac{1}{\sqrt{|S_u||S_v|}}\right)^{\frac{2}{n(n-1)}} \\
  (\text{Each } u \in V \text{ appears in exactly } n - 1 \text{ edges}) &= |E| \left(\left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{(n-1)/2}\right)^{\frac{2}{n(n-1)}} \\
  &= |E| \left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{1/n},
\end{align*}
which implies that $P(1)$ is true as desired.

\Ruizhe{
In our setting, the expected value is
\begin{align*}
    val(\varphi) = \sum_{i,j=1}^n \binom{k}{A_{i,j}}\binom{r-k}{k-A_{i,j}}\binom{r}{k}^{-1}.
\end{align*}
}

\paragraph{Inductive Step.} Let $j$ be any positive integer. Suppose that $P(j)$ holds.

We will now describe {\textsc{Approx-CompleteGame}$_{j+1}$} based on {\textsc{Approx-CompleteGame}$_j$} as follows.

\iffalse
\Zhao{We can hard code the algorithm}
\begin{algorithm}[h]\caption{\Zhao{Do we need to change the name of algorithm?}}
\begin{algorithmic}[1]
\Procedure{$\textsc{ApproxCompleteGame}_i(i > 0)$}{$\Sigma, V, E, \{C_{e}\}_{e \in E}, \{S_u\}_{u \in V}$}
    \State $R \leftarrow \left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{\frac{1}{n(j + 1)}}$.
    \While{true}
        \For{$u \in V$}
            \For{$v \in V$}
                \State $S_v^{u, \sigma_u} \leftarrow \{\sigma_v \in S_v \mid C_{(u, v)}(\sigma_u, \sigma_v) = 1\}$. 
                \State \Comment{Note that when $v = u$, let $S_u = \{\sigma_u\}$.} \label{step:reduce}
            \EndFor
            \If{$S_v^{u, \sigma_u} = \emptyset$ for some $v \in V$} 
                \State remove $\sigma_u$ from $S_u$ and continue to the next $u, \sigma_u$ pair. \label{step:empty}
            \EndIf
            \State $R^{u, \sigma_u} \leftarrow \left(\prod_{v \in V} \frac{1}{|S_v^{u, \sigma_u}|}\right)^{\frac{1}{nj}}$.
            \If{$R' < R$} 
                \State continue to the next $u, \sigma_u$ pair.
            \EndIf
            \State $\varphi \leftarrow$ {\sc Approx-CompleteGame$_j$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_v^{u, \sigma_u}\}_{v \in V}$). 
            \If{the output assignment is of value less than $R^{u, \sigma_u}$}
                \State remove $\sigma_u$ from $S_u$.
            \Else
                \State {\bf return} $\varphi$. \label{step:exc}
            \EndIf
        \EndFor
    \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi

\Zhao{if the following is an algorithm, please turn it into algoritihm template}
\begin{enumerate}
\item Define $R$ to be $\left(\prod_{u \in V} \frac{1}{|S_u|}\right)^{\frac{1}{n(j + 1)}}$, our target value we want to achieve.
\item Run the following steps~\ref{step:reduce} to~\ref{step:exc} until no $S_u$ is modified by neither step~\ref{step:exc} nor step~\ref{step:empty}.
  \begin{enumerate}
  \item For each $u \in V$ and $\sigma_u \in S_u$, do the following:
    \begin{enumerate}
    \item For each $v \in V$, compute $S_v^{u, \sigma_u} = \{\sigma_v \in S_v \mid C_{(u, v)}(\sigma_u, \sigma_v) = 1\}$. This is the set of reduced assignments of $v$ if we assign $\sigma_u$ to $u$. Note that when $v = u$, let $S_u = \{\sigma_u\}$. \label{step:reduce}
    \item If $S_v^{u, \sigma_u} = \emptyset$ for some $v \in V$, then remove $\sigma_u$ from $S_u$ and continue to the next $u, \sigma_u$ pair. \label{step:empty}
    \item Compute $R^{u, \sigma_u} = \left(\prod_{v \in V} \frac{1}{|S_v^{u, \sigma_u}|}\right)^{\frac{1}{nj}}$. If $R' < R$, continue to the next $u, \sigma_u$ pair.
    \item Execute {\sc Approx-CompleteGame$_j$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_v^{u, \sigma_u}\}_{v \in V}$). If the output assignment is of value less than $R^{u, \sigma_u}$, then remove $\sigma_u$ from $S_u$. Otherwise, return the output assignment as the output to {\sc Approx-CompleteGame$_{j+1}$}. \label{step:exc}
    \end{enumerate}
  \end{enumerate}
\item If the loop in the previous step ends without outputting any assignment, just output a random assignment (i.e. pick $\varphi(u)$ independently and uniformly at random from $S_u$). \label{step:random-assignment}
\end{enumerate}

Observe first that the loop can run at most $nq$ times as the total number of elements of $S_v$'s for all $v \in V$ is at most $nq$. This means that we call {\sc Approx-CompleteGame$_{j}$} at most $nq$ times. Since every step except the {\sc Approx-CompleteGame$_{j}$} calls takes $O((nq)^3)$ time and we call {\sc Approx-CompleteGame$_{j}$} only at most $n^2q^2$ times, we can conclude that the running time of {\sc Approx-CompleteGame$_{j+1}$} is $O((nq)^{3j+3})$ as desired.

The only thing left to show is that the assignment output from the algorithm indeed is of expected value at least $R$. To do so, we will consider two cases.

First, if step~\ref{step:random-assignment} is never reached, the algorithm must terminate at step~\ref{step:exc}. From the return condition in step~\ref{step:exc}, we know that the output assignment is of value at least $R^{u, \sigma_u} \geq R$ as desired.

In the second case where step~\ref{step:random-assignment} is reached, we first observe that when we remove $s_u$ from $S_u$ in step~\ref{step:exc}, the instance is still satisfiable. The reason is that, if $\sigma_u = \sigma_u^{\OPT}$ is the optimal assignment for $u$, then $\sigma_v^{\OPT}$ remains in $S_v^{u, \sigma_u}$ for every $v \in V$. Hence, from our inductive hypothesis, the output assignment from {\sc Approx-CompleteGame$_j$}($q, V, E, \{C_{e}\}_{e \in E}, \{S_v^{u, \sigma_u}\}_{v \in V}$) must be of value at least $R^{u, \sigma_u}$. As a result, we never remove $s^{\OPT}_u$ from $S_u$, and, thus, the instance remains satisfiable throughout the algorithm.

Moreover, notice that, if $R^{u, \sigma_u} \geq R$ for any $u, \sigma_u$, we either remove $\sigma_u$ from $S_u$ or output the desired assignment. This means that, when step~\ref{step:random-assignment} is reached, $R^{u, \sigma_u} < R$ for every $u \in V$ and $\sigma_u \in S_u$.

Now, let us consider the expected number of edges satisfied by the random assignment. Since our graph $(V, E)$ is complete, it can be written as follows.

\begin{align*}
  \mathbb{E} [\sum_{(u, v) \in E} C_{(u, v)}(\varphi(u), \varphi(v)) ] &= \mathbb{E} [\frac{1}{2}\sum_{u \in V} \sum_{v \in V \backslash \{u\} } C_{(u, v)}(\varphi(u), \varphi(v)) ] \\
  &= \frac{1}{2}\sum_{u \in V} \sum_{ v \in V \backslash \{ u \} } \mathbb{E}\left[C_{(u, v)}(\varphi(u), \varphi(v))\right] \\
  &= \frac{1}{2}\sum_{u \in V} \sum_{ v \in V \backslash \{ u \} } \frac{1}{|S_u||S_v|} \left(\sum_{\sigma_u \in S_u} \sum_{\sigma_v \in S_v} C_{(u, v)}(\sigma_u, \sigma_v)\right) \\
   &= \frac{1}{2}\sum_{u \in V} \sum_{ v \in V \backslash \{ u \} } \frac{1}{|S_u||S_v|} \left(\sum_{\sigma_u \in S_u} |S_v^{u, \sigma_u}|\right) \\
  &= \frac{1}{2} \sum_{u \in V} \frac{1}{|S_u|} \sum_{\sigma_u \in S_u}  (\sum_{ v \in V \backslash \{ u \} } \frac{|S_v^{u, \sigma_u}|}{|S_v|} ) 
\end{align*}
where the forth step follows from definition of $S_v^{u, \sigma_u}$.

\begin{align*}
 \E[\sum_{(u, v) \in E} C_{(u, v)}(\varphi(u), \varphi(v))] &\geq \sum_{u \in V_L} \frac{1}{|S_u|} \sum_{\sigma_u \in S_u} \left(\sum_{v \in V_R} \frac{|S_v^{u, \sigma_u}|}{|S_v|}\right) \\
  &\geq \sum_{u \in V_L} \frac{1}{|S_u|} \sum_{\sigma_u \in S_u} n \frac{(\prod_{v \in V_R}|S_v^{u, \sigma_u}|)^{1/n}}{(\prod_{v \in V_R}|S_v|)^{1/n}} \\
 &= n\left(\prod_{v\in V_R}|S_v|\right)^{-1/n} \sum_{u \in V_L} \frac{1}{|S_u|} \sum_{\sigma_u \in S_u} \left(\prod_{v \in V_R} |S_v^{u, \sigma_u}|\right)^{1/n}.
\end{align*}
By symmetry, we also have
\begin{align*}
    \E[\sum_{(u, v) \in E} C_{(u, v)}(\varphi(u), \varphi(v))] \geq n\left(\prod_{v\in V_L}|S_v|\right)^{-1/n} \sum_{u \in V_R} \frac{1}{|S_u|} \sum_{\sigma_u \in S_u} \left(\prod_{v \in V_L} |S_v^{u, \sigma_u}|\right)^{1/n}.
\end{align*}
Hence,
\begin{align*}
    \E[\sum_{(u, v) \in E} C_{(u, v)}(\varphi(u), \varphi(v))]^2 \geq n\left(\prod_{v\in V_L\cup V_R}|S_v|\right)^{-1/n} \sum_{u \in V_L}\sum_{v\in V_R} \frac{1}{|S_u||S_v|} \sum_{\sigma_u \in S_u,\sigma_v\in S_v} \left(\prod_{v \in V_L\cup V_R} |S_v^{u, \sigma_u}|\right)^{1/n}
\end{align*}
By definition of $R$ and $R^{u,\sigma}$, $(\prod_{v\in V_L\cup V_R}|S_v|)^{-1/n} = R^{(j+1)^2/2}$, $(\prod_{v \in V_L\cup V_R} |S_v^{u, \sigma_u}|)^{1/n} = (R^{u,\sigma_u})^{-j^2/2}$. Hence,


Since $\frac{n(n-1)}{2}$ is the number of edges in $(V, E)$, we can conclude that the random assignment is indeed of expected value at least $R$.

Thus, we can conclude that $P(j + 1)$ is true. As a result, $P(i)$ is true for every positive integer $i$, which completes the proof for Lemma~\ref{lem:approx-complete-game}.
\end{proof}

Next, we will prove Corollary~\ref{cor:qptas-dense} by reducing it to {\sc Max 2-CSP} on complete graph, and, then plug in Lemma~\ref{lem:approx-complete-game} with appropriate $i$ to get the result.

First, observe that, since $\log(1 + \varepsilon') = \Omega(\varepsilon')$ for every $1 \geq \varepsilon' > 0$, by plugging in $i = C \log q/\varepsilon'$ for large enough constant $C$ into Lemma~\ref{lem:approx-complete-game}, we immediately arrive the following corollary. \\

\begin{corollary} \label{cor:qptas-complete}
  For any $1 \geq \varepsilon' > 0$, there exists an $(1 + \varepsilon')$-approximation algorithm for satisfiable {\sc Max 2-CSP} on the complete graph that runs in time $N^{O(\varepsilon'^{-1}\log N)}$.
\end{corollary}

\begin{corollary}[QPTAS for Dense {Max 2-CSP}] \label{cor:qptas-dense}
  For any $1 \geq \varepsilon > 0$, there exists an $(1 + \varepsilon)$-approximation algorithm for satisfiable $\delta$-dense {\sc Max 2-CSP} that runs in time $N^{O(\varepsilon^{-1}\delta^{-1}\log N)}$.
\end{corollary}

Now, we will proceed to show the reduction and, thus, prove Corollary~\ref{cor:qptas-dense}.

\begin{proof}[Proof of Corollary~\ref{cor:qptas-dense}]
  First of all, notice that, since $\frac{1}{1 + \varepsilon} = 1 - \Theta(\varepsilon)$. It is enough for us to show that there exists an $N^{O(\varepsilon^{-1}\delta^{-1}\log N)}$-time algorithm for satisfiable $\delta$-dense {\sc Max 2-CSP} that produces an assignment of value at least $1 - \varepsilon$.

  On input $(q, V, E, \{C_e\}_{e \in E})$, the algorithm works as follows:
  \begin{enumerate}
    \item Construct a {\sc Max 2-CSP} instance $(q, V, E', \{C'_e\}_{e \in E'})$ where $(V, E')$ is a complete graph and $C'_e$ is defined as $C_e$ if $e \in E$. Otherwise, $C_e := 1$. In other words, we put in dummy constraints that are always true just to make the graph complete.
    \item Run the algorithm from Corollary~\ref{cor:qptas-complete} on $(q, V, E', \{C'_e\}_{e \in E'})$ with $\varepsilon' = \varepsilon \delta$ and output the assignment got from the algorithm.
  \end{enumerate}

  To see that the algorithm indeed produces an assignment with value $1 - \varepsilon$ for the input instance, first observe that, since $(q, V, E, \{C_e\}_{e \in E})$ is satisfiable,  $(q, V, E', \{C'_e\}_{e \in E'})$ is trivially satisfiable. Thus, from Corollary~\ref{cor:qptas-complete}, the output assignment has value at least $1/(1 + \delta\varepsilon) \geq 1 - \delta \varepsilon$ with respect to $(q, V, E', \{C'_e\}_{e \in E'})$. In other words, the assignment does not satisfy at most $\delta \varepsilon n^2$ edges. Thus, with respect to the input instance, it satisfies at least $\delta n^2 - \delta \varepsilon n^2 = (1 - \varepsilon) \delta n^2$ edges. In other words, it is of value at least $1 - \varepsilon$ as desired.

  Lastly, note that the running time of this algorithm is determined by that of the algorithm from Corollary~\ref{cor:qptas-complete}, which runs in $N^{O(\varepsilon'^{-1}\log N)} = N^{O(\varepsilon^{-1}\delta^{-1}\log N)}$ time as desired.
\end{proof}



\begin{comment}
\subsection{\cite{y14}'s Algorithm}

\begin{definition}[Critical constraints]
For $v\in [n]$ and $S\subseteq [n]$, for any partial assignment $\sigma_S: S\rightarrow [q]$, the set of critical constraints for $v$ and $\sigma_S$ is defined as follows:
\begin{align*}
    \mathsf{Crit}(v, S) := \{(v,u)\in \mathcal{C}: (v,u) ~\text{is not satisfied by}~\sigma_S\},
\end{align*}
where $\mathcal{C}$ is the set of constraints of the 2-CSP instance.
\end{definition}

\begin{definition}[Partial value]
Given a 2-CSP instance $([n], \mathcal{C}, [q])$. For a partial assignment $\sigma: S\rightarrow [q]$ where $S\subseteq [n]$, the value with respect to a set $T\subseteq [n]$ is defined as
\begin{align*}
    \mathsf{val}(\sigma, T) := |\{(u,v)\in \mathcal{C}: u,v\in T, (u,v)~\text{satisfied by}~\sigma\}|,
\end{align*}
where $(u,v)\in \mathcal{C}$ means there is a constraint on variables $u$ and $v$.
\Zhao{Do you mean $\sigma(u) = v$?}
\end{definition}
\iffalse

\begin{algorithm}[H]
    \caption{Two-Step Subsampling PTAS. The running time of this algorithm is $O(n q^4 \epsilon^{-2}) + 2^{O(\epsilon^{-1} \log q)} $ claimed by \cite{y14}. We are NOT sure about the analysis of the correctness of this algorithm. }\label{alg:ptas-rcsp}
    \begin{algorithmic}[1]
    \State \textbf{Input:} A $2$-CSP instance over $n$ variables, constraints set $\mathcal{C}$, alphabet size $q$, parameter $\epsilon$.
    \State \textbf{Output:} An assignment $\tau:[n]\rightarrow [q]$ such that $\mathsf{val}(\tau, [n])\geq \mathrm{OPT} - \epsilon n^2$.
    \State
    \Procedure{\textsc{GreedyAssign}}{$S_0, S_1, \sigma$} \Comment{$|S_1|n^{2/3}
    q^5\epsilon^{-2}$}
    \State \Comment{This procedure extends the partial assignment $\sigma:S_0\rightarrow [q]$ to $S_1$.}
        \State \Comment{$\sigma : S_0 \rightarrow [q]$}
        \State Randomly shuffle $S_1 \setminus S_0$ 
        \ForAll {$v \in S_1 \setminus S_0$}  \Comment{Each iteration takes $O(wq)$-time}
            \State $w\leftarrow O\left((n/|S_0|)^{2/3}q^4\epsilon^{-2}\right)$ \Comment{$w \in [n]$}
            \State Pick $D$ from $\binom{S_0}{w}$ uniformly at random \Comment{Runs in $O(w)$-time}
            \State $\mathsf{Crit}(v,D)\leftarrow \emptyset$
            \For{$u \in D$} \Comment{Runs in $O(w)$-time}
                \If{$ C_{(v,u)}\in \mathcal{C} $}
                    \State $\mathsf{Crit}(v,D)\leftarrow \mathsf{Crit}(v, D) \cup \{u\}$  
             \EndIf
            \EndFor
            \State $\sigma(v)\leftarrow \arg \max_{i\in [q]} ~\big|\{u\in \mathsf{Crit}(v,D): C_{(v,u)}(i, \sigma(u))=1\}\big|$. \Comment{Runs in $O(wq)$-time} %\Zhao{Why is this line define, but not assign?}
            \State $S_0 \leftarrow S_0 \cup \{v\}$ .
        \EndFor
        \State \Return $\sigma$ \Comment{$\sigma : S_1 \rightarrow [q]$}
    \EndProcedure
    \State
    \Procedure{\textsc{Main}}{}
        \State \Comment{What is the meaning of notation $\in_u$?}
        \State Pick $S_1\in_u \binom{[n]}{t_1}$ where $t_1 = O(\log^2 q / \epsilon^4)$
        \State Pick $S_0 \in_u  \binom{S_1}{t_0}$ where $t_0 = 1/\epsilon^2$.
        \State $\tau(v)\leftarrow 0$ for all $v\in [n]$
        \ForAll {partial assignment $\sigma:S_0\rightarrow [q]$} \Comment{$q^{|S_0|}$ times}\label{ln:first-loop} 
            \State $\sigma\leftarrow \textsc{GreedyAssign}(S_0, S_1, \sigma)$
            \If{$\mathsf{val}(\sigma, S_1)>\mathsf{val}(\tau,S_1)$}
                \State $\tau \leftarrow  \sigma$
            \EndIf
        \EndFor
        \State $\tau\leftarrow \textsc{GreedyAssign}(S_1, [n], \tau)$
        
        \State \Return $\tau$
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
\fi

\begin{theorem}[Theorem 1.2 in \cite{y14}]\label{thm:theorem_1.2_in_y14}
Algorithm~\ref{alg:ptas-rcsp} can approximate any 2-CSP problem over alphabet of size $q$ and $n$ variables within additive error $O(\epsilon n^2)$ and runs in time $O(nq^4\epsilon^{-2})+2^{O(\epsilon^{-1}\log q)}$.
\end{theorem}

\Ruizhe{The time complexity of Algorithm~\ref{alg:ptas-rcsp} is indeed  $O(nq^4\epsilon^{-2})+2^{O(\epsilon^{-1}\log q)}$, since the most time cost is in Line~\ref{ln:first-loop}, where we enumerate all partial assignment in time $q^{\epsilon^{-2}}$. The remaining parts can be done in $\poly(n,q)$.

Hence, I suspect that this algorithm is wrong.
}

\iffalse
\begin{algorithm}[H]
    \caption{One-Step Subsampling PTAS. (This is our guess and can match the running time mentioned in page 5 of footnote of \cite{mr17}, this is corresponding to max-cut alg in \cite{y14})}\label{alg:ptas-rcsp_one}

    \hspace*{\algorithmicindent} \textbf{Input:} A $2$-CSP instance over $n$ variables, constraints set $\mathcal{C}$, alphabet size $q$, parameter $\epsilon$.\\ 
    \hspace*{\algorithmicindent} \textbf{Output:} An assignment $\tau:[n]\rightarrow [q]$ such that $\mathsf{val}(\tau, [n])\geq \mathrm{OPT} - \epsilon n^2$.
    \begin{algorithmic}[1]
    \Procedure{\textsc{Main}}{}
        \State Pick $S_1\in_u \binom{[n]}{t_1}$ where $t_1 = O(\log q / \epsilon^2)$.
        \State $\tau(v)\leftarrow 0$ for all $v\in [n]$.
        \ForAll {partial assignment $\sigma:S_1\rightarrow [q]$}\label{ln:first-loop} 
            \State $\sigma\leftarrow \textsc{GreedyAssign}(S_1, [n], \sigma)$.
            \If{$\mathsf{val}(\sigma, [n])>\mathsf{val}(\tau,[n])$}
                \State $\tau \leftarrow  \sigma$.
            \EndIf
        \EndFor
        \State \Return $\tau$.
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
\fi

\begin{theorem}
Algorithm~\ref{alg:ptas-rcsp_one} can approximate any 2-CSP problem over alphabet of size $q$ and $n$ variables within additive error $O(\epsilon n^2)$ and runs in time $n\cdot q^{O(\epsilon^{-2}\log q)}$.
\end{theorem}

\Ruizhe{I guess Pasin verified that the above statement is correct. \cite{y14} used a similar algorithm to show that it works for Max-Cut. Maybe we (or Pasin) can prove that it also works for general Max 2-CSP.}
\end{comment}
\fi
